Mixture Reduction on Matrix Lie Groups

Many physical systems evolve on matrix Lie groups and mixture filtering designed for such manifolds represent an inevitable tool for challenging estimation problems. However, mixture filtering faces the issue of a constantly growing number of components, hence require appropriate mixture reduction techniques. In this letter we propose a mixture reduction approach for distributions on matrix Lie groups, called the concentrated Gaussian distributions (CGDs). This entails appropriate reparametrization of CGD parameters to compute the KL divergence, pick and merge the mixture components. Furthermore, we also introduce a multitarget tracking filter on Lie groups as a mixture filtering study example for the proposed reduction method. In particular, we implemented the probability hypothesis density filter on matrix Lie groups. We validate the filter performance using the optimal subpattern assignment metric on a synthetic dataset consisting of 100 randomly generated multitarget scenarios.

==> figures/statistics.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.34667,0.53600,0.69067}%
\definecolor{mycolor2}{rgb}{0.91529,0.28157,0.28784}%
\definecolor{mycolor3}{rgb}{0.44157,0.74902,0.43216}%
\definecolor{mycolor4}{rgb}{1.00000,0.59843,0.20000}%
\definecolor{mycolor5}{rgb}{0.67686,0.44471,0.71137}%
%
\begin{tikzpicture}

\begin{axis}[%
compat=newest,
width=0.4\columnwidth,
height=1.2in,
scale only axis,
at={(-2.0in,1.5in)},
xmin=0.5,
xmax=5.5,
xtick={\empty},
ymin=57,
ymax=113,
xminorticks=true,
ylabel={Total OSPA [m]},
axis background/.style={fill=white},
title={Piecewise},
legend style={nodes=right},
legend pos=north west,
]
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	81.2084822625349\\
1	89.5044677903769\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	80.2649280313768\\
2	88.3740361953192\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	83.814646235311\\
3	93.2175973009229\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	83.7757494794779\\
4	92.9680098816959\\
};
\addplot [color=mycolor5,dashed,forget plot]
  table[row sep=crcr]{%
5	83.188191297811\\
5	89.5352491403511\\
};
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	58.8846431057492\\
1	67.7657700578831\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	60.7189123603974\\
2	68.1426469913782\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	60.7481111245167\\
3	70.3306534813918\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	58.4919622217468\\
4	70.3574527764332\\
};
\addplot [color=mycolor5,dashed,forget plot]
  table[row sep=crcr]{%
5	62.1906731162311\\
5	69.2948617228564\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	89.5044677903769\\
1.125	89.5044677903769\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	88.3740361953192\\
2.125	88.3740361953192\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	93.2175973009229\\
3.125	93.2175973009229\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	92.9680098816959\\
4.125	92.9680098816959\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.875	89.5352491403511\\
5.125	89.5352491403511\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	58.8846431057492\\
1.125	58.8846431057492\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	60.7189123603974\\
2.125	60.7189123603974\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	60.7481111245167\\
3.125	60.7481111245167\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	58.4919622217468\\
4.125	58.4919622217468\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.875	62.1906731162311\\
5.125	62.1906731162311\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	67.7657700578831\\
0.75	81.2084822625349\\
1.25	81.2084822625349\\
1.25	67.7657700578831\\
0.75	67.7657700578831\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	68.1426469913782\\
1.75	80.2649280313768\\
2.25	80.2649280313768\\
2.25	68.1426469913782\\
1.75	68.1426469913782\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	70.3306534813918\\
2.75	83.814646235311\\
3.25	83.814646235311\\
3.25	70.3306534813918\\
2.75	70.3306534813918\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	70.3574527764332\\
3.75	83.7757494794779\\
4.25	83.7757494794779\\
4.25	70.3574527764332\\
3.75	70.3574527764332\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.75	69.2948617228564\\
4.75	83.188191297811\\
5.25	83.188191297811\\
5.25	69.2948617228564\\
4.75	69.2948617228564\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	75.339744795493\\
1.25	75.339744795493\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	73.1832393133206\\
2.25	73.1832393133206\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	76.6548929877867\\
3.25	76.6548929877867\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	75.2432117628253\\
4.25	75.2432117628253\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.75	76.6752498785929\\
5.25	76.6752498785929\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=blue,line width=1.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
1	74.1196770635079\\
2	73.6459026900191\\
3	77.1044863285954\\
4	76.7636404916508\\
5	76.3524400451362\\
};
\end{axis}

\begin{axis}[%
compat=newest,
width=0.4\columnwidth,
height=1.2in,
at={(-2.0in,0.2in)},
scale only axis,
xmin=0.5,
xmax=5.5,
xtick={\empty},
ymin=45,
ymax=90,
xminorticks=true,
ylabel={Distance OSPA [m]},
axis background/.style={fill=white},
legend style={nodes=right},
legend pos=north west,
]
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	59.3613341188657\\
1	64.1080491026146\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	59.1844198284398\\
2	63.0812479061663\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	62.4493725079611\\
3	70.1607704806577\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	62.9091614236664\\
4	69.3447142332442\\
};
\addplot [color=mycolor5,dashed,forget plot]
  table[row sep=crcr]{%
5	61.6080903335307\\
5	66.422424074179\\
};
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	46.0988686723153\\
1	50.1999156854591\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	47.2211466021009\\
2	50.6758745576324\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	47.9600095630947\\
3	53.332556311481\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	45.7038671636115\\
4	51.4691798870412\\
};
\addplot [color=mycolor5,dashed,forget plot]
  table[row sep=crcr]{%
5	48.4611963371426\\
5	52.6532652211069\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	64.1080491026146\\
1.125	64.1080491026146\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	63.0812479061663\\
2.125	63.0812479061663\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	70.1607704806577\\
3.125	70.1607704806577\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	69.3447142332442\\
4.125	69.3447142332442\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.875	66.422424074179\\
5.125	66.422424074179\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	46.0988686723153\\
1.125	46.0988686723153\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	47.2211466021009\\
2.125	47.2211466021009\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	47.9600095630947\\
3.125	47.9600095630947\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	45.7038671636115\\
4.125	45.7038671636115\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.875	48.4611963371426\\
5.125	48.4611963371426\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	50.1999156854591\\
0.75	59.3613341188657\\
1.25	59.3613341188657\\
1.25	50.1999156854591\\
0.75	50.1999156854591\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	50.6758745576324\\
1.75	59.1844198284398\\
2.25	59.1844198284398\\
2.25	50.6758745576324\\
1.75	50.6758745576324\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	53.332556311481\\
2.75	62.4493725079611\\
3.25	62.4493725079611\\
3.25	53.332556311481\\
2.75	53.332556311481\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	51.4691798870412\\
3.75	62.9091614236664\\
4.25	62.9091614236664\\
4.25	51.4691798870412\\
3.75	51.4691798870412\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.75	52.6532652211069\\
4.75	61.6080903335307\\
5.25	61.6080903335307\\
5.25	52.6532652211069\\
4.75	52.6532652211069\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	53.6216803441948\\
1.25	53.6216803441948\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	53.9604017400395\\
2.25	53.9604017400395\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	57.7800264449617\\
3.25	57.7800264449617\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	57.2834908739959\\
4.25	57.2834908739959\\
};
\addplot [color=mycolor5,solid,forget plot]
  table[row sep=crcr]{%
4.75	58.443828112537\\
5.25	58.443828112537\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=blue,line width=1.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
1	54.788181211929\\
2	54.4157865699189\\
3	58.2725032807202\\
4	57.6495603170056\\
5	57.357562873433\\
};
\end{axis}


\begin{axis}[%
compat=newest,
width=0.4\columnwidth,
height=1.2in,
scale only axis,
at={(-0.2in,1.5in)},
xmin=0.5,
xmax=4.5,
xtick={\empty},
ymin=57,
ymax=113,
xminorticks=true,
ylabel={Total OSPA [m]},
axis background/.style={fill=white},
title={West},
legend style={nodes=right},
legend pos=north west,
]
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	99.2475909906428\\
1	103.546767191684\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	99.3017340973988\\
2	109.895496269534\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	101.793988390076\\
3	111.524757968402\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	97.1802309312679\\
4	110.263453364927\\
};
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	70.0919297858325\\
1	80.0471054661476\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	68.2742377484981\\
2	85.5657750557072\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	67.7396264169501\\
3	85.2979885720581\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	69.0621388216058\\
4	84.751202419454\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	103.546767191684\\
1.125	103.546767191684\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	109.895496269534\\
2.125	109.895496269534\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	111.524757968402\\
3.125	111.524757968402\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	110.263453364927\\
4.125	110.263453364927\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	70.0919297858325\\
1.125	70.0919297858325\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	68.2742377484981\\
2.125	68.2742377484981\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	67.7396264169501\\
3.125	67.7396264169501\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	69.0621388216058\\
4.125	69.0621388216058\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	80.0471054661476\\
0.75	99.2475909906428\\
1.25	99.2475909906428\\
1.25	80.0471054661476\\
0.75	80.0471054661476\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	85.5657750557072\\
1.75	99.3017340973988\\
2.25	99.3017340973988\\
2.25	85.5657750557072\\
1.75	85.5657750557072\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	85.2979885720581\\
2.75	101.793988390076\\
3.25	101.793988390076\\
3.25	85.2979885720581\\
2.75	85.2979885720581\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	84.751202419454\\
3.75	97.1802309312679\\
4.25	97.1802309312679\\
4.25	84.751202419454\\
3.75	84.751202419454\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	90.605543711817\\
1.25	90.605543711817\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	90.6916754745722\\
2.25	90.6916754745722\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	89.2518801574268\\
3.25	89.2518801574268\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	89.9003113390864\\
4.25	89.9003113390864\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
2	64.0322455888873\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=blue,line width=1.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
1	88.9707535972203\\
2	89.9180861194337\\
3	91.9342640084394\\
4	91.1348264443589\\
};
\end{axis}

\begin{axis}[%
compat=newest,
width=0.4\columnwidth,
height=1.2in,
at={(-0.2in,0.2in)},
scale only axis,
xmin=0.5,
xmax=4.5,
xtick={\empty},
ymin=45,
ymax=90,
xminorticks=true,
yminorticks=true,
ylabel={Distance OSPA [m]},
axis background/.style={fill=white},
legend style={nodes=right},
legend pos=north west,
]
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	73.0228895320607\\
1	85.3080049898661\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	74.8177533949881\\
2	82.7292617731898\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	76.4620849738978\\
3	88.8734292378979\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	74.6998480700781\\
4	91.1185653163944\\
};
\addplot [color=mycolor1,dashed,forget plot]
  table[row sep=crcr]{%
1	53.3026009639428\\
1	61.8499413817868\\
};
\addplot [color=mycolor2,dashed,forget plot]
  table[row sep=crcr]{%
2	51.8053123516551\\
2	63.5349437932441\\
};
\addplot [color=mycolor3,dashed,forget plot]
  table[row sep=crcr]{%
3	51.9183755689131\\
3	64.241571416265\\
};
\addplot [color=mycolor4,dashed,forget plot]
  table[row sep=crcr]{%
4	58.4229462687595\\
4	62.3111691093474\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	85.3080049898661\\
1.125	85.3080049898661\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	82.7292617731898\\
2.125	82.7292617731898\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	88.8734292378979\\
3.125	88.8734292378979\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	91.1185653163944\\
4.125	91.1185653163944\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.875	53.3026009639428\\
1.125	53.3026009639428\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.875	51.8053123516551\\
2.125	51.8053123516551\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.875	51.9183755689131\\
3.125	51.9183755689131\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.875	58.4229462687595\\
4.125	58.4229462687595\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	61.8499413817868\\
0.75	73.0228895320607\\
1.25	73.0228895320607\\
1.25	61.8499413817868\\
0.75	61.8499413817868\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	63.5349437932441\\
1.75	74.8177533949881\\
2.25	74.8177533949881\\
2.25	63.5349437932441\\
1.75	63.5349437932441\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	64.241571416265\\
2.75	76.4620849738978\\
3.25	76.4620849738978\\
3.25	64.241571416265\\
2.75	64.241571416265\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	62.3111691093474\\
3.75	74.6998480700781\\
4.25	74.6998480700781\\
4.25	62.3111691093474\\
3.75	62.3111691093474\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0.75	64.3411120564277\\
1.25	64.3411120564277\\
};
\addplot [color=mycolor2,solid,forget plot]
  table[row sep=crcr]{%
1.75	67.9201968883066\\
2.25	67.9201968883066\\
};
\addplot [color=mycolor3,solid,forget plot]
  table[row sep=crcr]{%
2.75	70.0869848635723\\
3.25	70.0869848635723\\
};
\addplot [color=mycolor4,solid,forget plot]
  table[row sep=crcr]{%
3.75	67.3876745109237\\
4.25	67.3876745109237\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=asterisk,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=blue,line width=1.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
1	67.7141559394778\\
2	68.3565525090443\\
3	70.7889082410347\\
4	69.741086341242\\
};
\end{axis}

\end{tikzpicture}%
